Detection of UHE gamma rays from the Crab Nebula: Physical Implications

The Crab Nebula is an extreme particle accelerator boosting the energy of electrons up to a few PeV ($10^{15} \ \rm eV$), close to the maximum energy allowed by theory. The physical conditions in the acceleration site and the nature of the acceleration process itself remain highly uncertain. The key information about the highest energy accelerated particles is contained in the synchrotron and inverse Compton (IC) channels of radiation at energies above 1~MeV and 100~TeV, respectively. The recent report of detection of ultra-high energy gamma-ray signal from the Crab Nebula up to 300~TeV allows one to determine the energy distribution of the highest energy electrons and to derive the magnetic field strength in the acceleration region, $B\leq120\rm\,\mu G$, in a parameter-free way. This estimate brings new constraints on the properties of non-thermal particle distributions and puts important constraints on the MHD models for the Crab Nebula, in particular on the feasible magnetization and anisotropy of the pulsar wind. The calculations of synchrotron and IC emission show that future observations with instruments allowing detection of the Crab Nebula above 300~TeV and above 1~MeV will clarify the conditions allowing acceleration of electrons beyond PeV energies in the Crab Nebula. In particular, one will (1) verify the hypothetical multi-component composition of the electron energy distribution, and (2) determine the magnetic field strength in the regions responsible for the acceleration of PeV electrons.

==> myacro.tex <==
\usepackage[single=true]{acro}
% objects
\DeclareAcronym{agn}{
  short = AGN,
  long  = active galactic nucleus,
  short-plural = s,
  long-plural-form = active galactic nuclei,
  class = astro,
  first-style = default
}
\DeclareAcronym{smbh}{
  short = SMBH ,
  long  = supermassive black hole ,
  class = astro ,
  first-style = default
}
\DeclareAcronym{pwn}{
  short = PWN ,
  long  = pulsar wind nebula ,
  short-plural = e ,
  long-plural = e ,
  class = astro ,
  first-style = default
}
\DeclareAcronym{cr}{
  short = CR ,
  long  = cosmic ray ,
  class = astro ,
  first-style = default
}
\DeclareAcronym{ns}{
  short = NS ,
  long  = neutron star ,
  class = astro ,
  first-style = default
}
\DeclareAcronym{ism}{
  short = ISM ,
  long  = interstellar medium ,
  class = astro ,
  first-style = default
}

\DeclareAcronym{cmbr}{
  short = CMBR ,
  long  = Cosmic Microwave Background Radiation ,
  class = astro,
  first-style = default
}
\DeclareAcronym{ebl}{
  short = EBL ,
  long  = extragalactic background light ,
  class = astro,
  first-style = default
}
\DeclareAcronym{fir}{
  short = FIR ,
  long  = far-infrared ,
  class = astro,
  first-style = default
}
\DeclareAcronym{nir}{
  short = NIR ,
  long  = near-infrared ,
  class = astro,
  first-style = default
}
% processes
\DeclareAcronym{dsa}{
  short = DSA ,
  long  = diffusive shock acceleration ,
  class = astro ,
  first-style = default
}
\DeclareAcronym{sto}{
  short = StA ,
  long  = stochastic acceleration ,
  class = astro ,
  first-style = default
}
\DeclareAcronym{ic}{
  short = IC ,
  long  = inverse Compton ,
  class = astro ,
  first-style = default
}
\DeclareAcronym{ssa}{
  short = SSA ,
  long  = synchrotron-self-abosrption ,
  class = astro ,
  first-style = default
}
\DeclareAcronym{ssc}{
  short = SSC ,
  long  = synchrotron-self-Compton ,
  class = astro ,
  first-style = default
}
\DeclareAcronym{kn}{
  short = KN ,
  long  = Klein~--~Nishina ,
  class = astro ,
  first-style = default
}
\DeclareAcronym{ec}{
  short = EC ,
  long  = elastic Coulomb ,
  class = astro ,
  first-style = default
}
\DeclareAcronym{pp}{
  short = \ensuremath{pp} ,
  long  = hadronuclear ,
  class = astro ,
  first-style = default
}
\DeclareAcronym{pg}{
  short = \ensuremath{p\gamma} ,
  long  = photomeson ,
  class = astro ,
  first-style = default
}

%  emission
\DeclareAcronym{he}{
  short = \aciffirst{HE, \(>100\) MeV}{HE} ,
  short-plural-form = \aciffirst{HE, \(>100\) MeV}{HE} ,
  long  = high-energy ,
  long-plural-form = high energies ,
  class = hydro ,
  first-style = default
}
\DeclareAcronym{vhe}{
  short = \aciffirst{VHE, \(>100\) GeV}{VHE} ,
  short-plural-form = \aciffirst{VHE, \(>100\) GeV}{VHE} ,
  long  = very high-energy ,
  class = astro ,
  first-style = default 
}
\DeclareAcronym{uhe}{
  short = \aciffirst{UHE, \(>100\) TeV}{UHE} ,
  short-plural-form = \aciffirst{UHE, \(>100\) TeV}{UHE} ,
  long  = ultra high-energy ,
  class = astro ,
  first-style = default 
}
\DeclareAcronym{sed}{
  short = SED ,
  long  = Spectral Energy Distribution ,
  single  = spectral energy distribution ,
  class = astro ,
  first-style = default
}
\DeclareAcronym{mec}{
  short = MEC ,
  long  = monochromatic emission coefficient ,
  class = astro ,
  first-style = default
}

% hydro
\DeclareAcronym{hd}{
  short = HD ,
  long  = hydrodynamic ,
  class = hydro ,
  first-style = default 
}

\DeclareAcronym{mhd}{
  short = MHD ,
  long  = \acifused{hd}{magneto-HD}{magnetohydrodynamic} ,
  class = hydro ,
  first-style = default 
}
\DeclareAcronym{rmhd}{
  short = RMHD ,
  long  = \acifused{mhd}{relativistic MHD}{\acifused{hd}{relativistic magneto HD}{relativistic magnetohydrodynamic}} ,
  class = hydro ,
  first-style = default
}
\DeclareAcronym{1d}{
  short = \aciffirst{1D\footnote{We use the standard abbreviation ``ND'' for N-dimensional.\acuse{2d,3d}}}{1D} ,
  long  = one-dimensional ,
  class = hydro ,
  first-style = short
}
\DeclareAcronym{2d}{
  short = \aciffirst{2D\footnote{We use the standard abbreviation ``ND'' for N-dimensional.\acuse{1d,3d}}}{2D} ,
  long  = two-dimensional ,
  class = hydro ,
  first-style = short
}
\DeclareAcronym{3d}{
  short = \aciffirst{3D\footnote{We use the standard abbreviation ``ND'' for N-dimensional.\acuse{1d,2d}}}{3D} ,
  long  = three-dimensional ,
  class = hydro ,
  first-style = short
}
\DeclareAcronym{cd}{
  short = CD ,
  long  = contact discontinuity ,
  class = hydro ,
  first-style = default
}
\DeclareAcronym{ts}{
  short = TS ,
  long  = termination shock ,
  class = hydro ,
  first-style = default
}
\DeclareAcronym{eos}{
  short = EOS ,
  long  =  equation of state ,
  long-plural-form = equations of state ,
  class = hydro ,
  first-style = default
}

\DeclareAcronym{pic}{
  short = PIC ,
  long = particle-in-cell ,
  first-style = default
}
\DeclareAcronym{mcmc}{
  short = MCMC ,
  long = Markov~Chain Monte~Carlo ,
  first-style = default
}

\DeclareAcronym{mq}{
  short = \(\upmu\)Q ,
  long = microquasar ,
  first-style = default
}


% instruments
\DeclareAcronym{alma}{
  short = ALMA ,
  long  = Atacama Large Millimeter/submillimeter Array ,
  class = instruments ,
  first-style = default
}
\DeclareAcronym{nustar}{
  short = {\it NuSTAR} ,
  long  = Nuclear Spectroscopic Telescope Array ,
  class = instruments ,
  first-style = default
}
\DeclareAcronym{integral}{
  short = {\it INTEGRAL} ,
  long  = {INTErnational Gamma-Ray Astrophysics Laboratory} ,
  single = {International Gamma-Ray Astrophysics Laboratory} ,
  class = instruments ,
  first-style = default
}
\DeclareAcronym{comptel}{
  short = {\it COMPTEL} ,
  long  = Imaging Compton Telescope ,
  class = instruments ,
  first-style = default
}
\DeclareAcronym{grams}{
  short = {\it GRAMS} ,
  long  = Gamma-Ray and AntiMatter Survey ,
  class = instruments ,
  first-style = default
}

\DeclareAcronym{fermi}{
  short = {\it Fermi}/LAT ,
  long  = {\it Fermi} Large Area Telescope ,
  class = instruments ,
  first-style = default
}
\DeclareAcronym{hegra}{
  short = HEGRA ,
  long  = High Energy Gamma Ray Astronomy ,
  class = instruments ,
  first-style = default
}
\DeclareAcronym{tibet}{
  short = {\it Tibet AS\(\gamma\)} ,
  long  = Tibet Air Show Gamma Experiment,
  class = instruments ,
  first-style = default
}
\DeclareAcronym{hawc}{
  short = {\it HAWC} ,
  long  = High Altitude Water Cherenkov Gamma-Ray Observatory ,
  class = instruments ,
  first-style = default
}

\DeclareAcronym{lhaaso}{
  short = {\it LHAASO} ,
  long  = Large High Altitude Air Shower Observatory ,
  class = instruments ,
  first-style = default
}


